A Revenue Function for Comparison-Based Hierarchical Clustering

Comparison-based learning addresses the problem of learning when, instead of explicit features or pairwise similarities, one only has access to comparisons of the form: \emph{Object $A$ is more similar to $B$ than to $C$.} Recently, it has been shown that, in Hierarchical Clustering, single and complete linkage can be directly implemented using only such comparisons while several algorithms have been proposed to emulate the behaviour of average linkage. Hence, finding hierarchies (or dendrograms) using only comparisons is a well understood problem. However, evaluating their meaningfulness when no ground-truth nor explicit similarities are available remains an open question. In this paper, we bridge this gap by proposing a new revenue function that allows one to measure the goodness of dendrograms using only comparisons. We show that this function is closely related to Dasgupta's cost for hierarchical clustering that uses pairwise similarities. On the theoretical side, we use the proposed revenue function to resolve the open problem of whether one can approximately recover a latent hierarchy using few triplet comparisons. On the practical side, we present principled algorithms for comparison-based hierarchical clustering based on the maximisation of the revenue and we empirically compare them with existing methods.

==> conjecture.tex <==
\section{Recovering Latent Hierarchy by Triplet Revenue Maximisation}
\label{sec:theory-latent}

In this section, we consider the problem of recovering a latent hierarchy from triplet comparisons, earlier studied in \citet{emamjomeh2018adaptive}.
Let $H_0$ be a hierarchy on $[n]$, from which we derive a set of triplets\footnote{%
\citet{emamjomeh2018adaptive} consider triples of the form $\{i,j,k\}$ that imply $i,j$ are closer to each other than $k$, with respect to $H_0$.  Each such triple $\{i,j,k\}$ correspond to two triplets $(i,j,k)$ and $(j,i,k)$ in our setting.}
\begin{displaymath}
\mathcal{T}_0 = \{(i,j,k), (j,i,k) ~:~ i,j \text{ are merged before } k \text{ in } H_0\}.
\end{displaymath}
One can show that any rooted tree $H'$ that satisfies all triplets in $\mathcal{T}_0$ is equivalent to $H_0$, up to isomorphic transformations, and hence, one can exactly recover $H_0$ given $\mathcal{T}_0$.
\citet{emamjomeh2018adaptive} further show one cannot exactly recover $H_0$ from any passively obtained $\mathcal{T} \subset \mathcal{T}_0$ if $|\mathcal{T}| = o(n^3)$.
This raises the question---can one approximately recover $H_0$ from a smaller set of triplets $\mathcal{T}$? 

To address this issue, we consider the setting where $\mathcal{T}_0$ is not completely available but one has access to a random subset $\mathcal{T} \subseteq \mathcal{T}_0$ obtained using the following strategy. Let $p_n \in (0,1]$ denote a sampling probability that depends on $n$ the number of objects. For every pair of triplets $(i,j,k),(j,i,k) \in \mathcal{T}_0$, we add the pair to $\mathcal{T}$ with probability $p_n$. One can then use standard concentration inequalities to show that, with high probability, $|\mathcal{T}| = O(p_n n^3)$. In the next theorem, we show that $|\mathcal{T}| = O(n^2 \log n) \ll n^3$ triplets sampled using this strategy suffice to obtain a tree $\widehat{H}$ whose revenue with respect to $\mathcal{T}_0$ is, in the worst case, only slightly lower than the the revenue of $H_0$.

\begin{theorem}
\label{thm-approx}
Let $p_n \in (0,1]$ that depends on $n$, and $\mathcal{T}$ be as defined above.
Given access to $\mathcal{T}$, consider the hierarchy 
\begin{displaymath}
\widehat{H} = \argmax_{H} Trev(H,\mathcal{T}).
\end{displaymath}
For any $\epsilon \in (0,1)$, there exist constants $n_0,c>0$ (depending on $\epsilon$) such that for $n> n_0$ and $p_n > c\log n/n$, 
\begin{equation}
?? \cdot Trev(H_0,\mathcal{T}_0) \geq Trev(\widehat{H},\mathcal{T}_0) \geq (1-\epsilon)\cdot Trev(H_0,\mathcal{T}_0)
\label{eqn-approx}
\end{equation}
with probability at least $1-n^{-O(1)}$. 
Setting $p_n$ at its smallest allowable value, \eqref{eqn-approx} holds for $|\mathcal{T}| = O(n^2 \log n)$.
\end{theorem}

\begin{proof}[Proof sketch (details in appendix)]
We use concentration inequalities to show that with probability $1-n^{-O(1)}$, for every tree $H$,
\begin{displaymath}
\big| Trev(H, \mathcal{T}) - p_n Trev(H,\mathcal{T}_0) \big| = O\left(n^3 \sqrt{p_n n\log n}\right).
\end{displaymath}
Using this concentration for both $H_0$ and $\widehat{H}$, and noting that $Trev(\widehat{H},\mathcal{T}) \geq Trev(H_0,\mathcal{T})$, we have
\begin{displaymath}
Trev(\widehat{H},\mathcal{T}_0) \geq Trev(H_0,\mathcal{T}_0) - O\left(\sqrt{\frac{n^7\log n}{p_n}}\right).
\end{displaymath}
Finally, we show that $Trev(H_0,\mathcal{T}_0) = \Omega(n^4)$ to arrive at the $(1-\epsilon)$-approximation for $p_n = \Omega(\log n/n)$.
\end{proof}
The result in \citet[][Proposition 2.2]{emamjomeh2018adaptive}---that $\Omega(n^3)$ triplets are necessary to exactly recover $H_0$---hinges on the fact that it is impossible to correctly guess the hierarchy at the lowest level of the tree $H_0$ using fewer comparisons.
Since errors in the lowest level do not significantly affect $Trev$, we can achieve the $(1-\epsilon)$-approximation in Theorem~\ref{thm-approx}. 

One of the limits of Theorem~\ref{thm-approx} is that it does not prevent the revenue of $\widehat{H}$ to be much higher that the revenue of $H_0$ implying that the two are potentially quite different. However, we believe that it is not the case and that $H_0$ is, in fact, the tree maximizing the revenue for the set of triplets $\mathcal{T}_0$. This is summarized in the next conjecture.

\begin{conjecture}
\label{thm-H0-maxrev}
Consider the aforementioned setting, where $H_0$ is a latent hierarchy on $[n]$ objects, and $\mathcal{T}_0$ is the set of corresponding triplets. Then
\begin{displaymath}
H_0 = \argmax_{H} Trev(H,\mathcal{T}_0),
\end{displaymath}
where the maximisation is over all binary trees $H$ on $[n]$.
\end{conjecture}

We can show that the conjecture holds for $n=3,4$ by doing an exhaustive list of all possible trees and verifying that the tree that maximizes the revenue for the set of triplets they generate is themselves. For example, given three objects $i,j,k$ the possible trees are:
\begin{itemize}
    \item[$H_k$]: Merge $i,j$ first and then $H(i\lor j)$ with $k$.
    \item[$H_j$]: Merge $i,k$ first and then $H(i\lor k)$ with $j$.
    \item[$H_i$]: Merge $j,k$ first and then $H(j\lor k)$ with $i$.
\end{itemize}
Without loss of generality, assume that $H_0 = H_k$, the corresponding set of triplets is $\mathcal{T}_0 = \left\{(i,j,k), (j,i,k) \right\}$. Then we have that $Trev(H_k,T_0) = 2$, $Trev(H_j,T_0) = -1$, and $Trev(H_i,T_0) = -1$.



Note that the uniqueness of the hierarchy that satisfies all triplets in $\mathcal{T}_0$ implies that $H_0$ maximises the function
\begin{displaymath}
f(H,\mathcal{T}_0) =\sum_{(i,j,k)\in\mathcal{T}_0} \mathbb{I}_{|H(i \lor k)| > |H(i \lor j)|}.
\end{displaymath}
While maximising $Trev(H,\mathcal{T}_0)$ seems to be a relaxation of maximising $f(H,\mathcal{T}_0)$ in this context, Conjecture~\ref{thm-H0-maxrev} would suggest that both problems have the same optimal solution $H_0$ and thus that maximizing the revenue is indeed a good way to find meaningful hierarchies. However, solving such a maximization problem is difficult in practice as it requires exhaustive search over all trees. We discuss practical algorithms in the next section.



==> removed-proofs.tex <==
\section{Original (longer) Proof of Theorem \ref{thm_equivalence} using induction}

The revenue function of the tree is defined as :
\[ Trev(H,\mathcal{T}) = \sum_{\substack{i,j,k \in \mathcal{T}}} \big[|H(i \lor k)| - |H(i \lor j)|\big]\]
This can also be written as : 
\[ Trev(H,\mathcal{V}) = \sum_{\substack{i,j,k \in \mathcal{V} \\ i \neq j \neq k}} \big[|H(i \lor k)| - |H(i \lor j)|\big]\mathbb{I} _{ij > ik}\]
Where $\mathcal{V}$ is the set of all nodes of tree H. The revenue can be represented in a different form as follows:
\begin{align*}
Trev(H,\mathcal{V}) = &\sum_{\substack{i,j \in \mathcal{V} \\ i \neq j }}|H(i \lor j)|\\&\sum_{\substack{k \in \mathcal{V}, k \neq i,j }}[\mathbb{I} _{ik > ij} - \mathbb{I} _{ij > ik} + \mathbb{I} _{jk > ij} - \mathbb{I} _{ij > jk}]
\end{align*}
This can be proved by induction. Taking three nodes i,j,k the cost can be simplified as shown below.
\begin{alignat*}{2}
Trev(H,\mathcal{V}) &= \big[|H(i \lor k)| - |H(i \lor j)|\big]\mathbb{I} _{ij > ki}\\ &+ \big[|H(j \lor k)| - |H(i \lor j)|\big]\mathbb{I} _{ij > jk}\\ &+ \big[|H(j \lor k)| - |H(k \lor i)|\big]\mathbb{I} _{ki > jk}\\ &+ \big[|H(i \lor j)| - |H(k \lor i)|\big]\mathbb{I} _{ki > ij} \\ &+ \big[|H(k \lor i)| - |H(j \lor k)|\big]\mathbb{I} _{jk > ki} \\ &+ \big[|H(i \lor j)| - |H(k \lor j)|\big]\mathbb{I} _{jk > ij}\\
&= |H(i \lor j)|\big[\mathbb{I} _{jk > ij} - \mathbb{I} _{ij > jk} + \mathbb{I} _{ki > ij} - \mathbb{I} _{ij > ki}\big]\\ &+ |H(j \lor k)|\big[\mathbb{I} _{ij > jk} - \mathbb{I} _{jk > ij} + \mathbb{I} _{ki > jk} - \mathbb{I} _{jk > ki}\big]\\
&+ |H(k \lor i)|\big[\mathbb{I} _{jk > ki} - \mathbb{I} _{ki > jk} + \mathbb{I} _{ij > ki} - \mathbb{I} _{ki > ij}\big]
\end{alignat*}
Let [n] denote the set containing n leaf nodes. The revenue of a tree containing n-1 leaves from the above equation is given below:
\begin{align*} 
Trev_{n-1}(H,[n-1]) &= \sum_{\substack{i,j \in [n-1] \\ i \neq j }}|H(i \lor j)|\\&\sum_{\substack{k \in [n-1] \\ k \neq i,j }}[\mathbb{I} _{ki > ij} - \mathbb{I} _{ij > ki} + \mathbb{I} _{jk > ij} - \mathbb{I} _{ij > jk}]
\end{align*}
Adding another node n, the revenue of the tree is as follows
\begin{align*}
&Trev_{n}(H,[n]) = \sum_{\substack{i,j \in [n-1] \\ i \neq j }}|H(i \lor j)|\\&\sum_{\substack{k \in [n-1] \\ k \neq i,j }}\big[\mathbb{I} _{ki > ij} - \mathbb{I} _{ij > ki} + \mathbb{I} _{jk > ij} - \mathbb{I} _{ij > jk}\big]\\ 
&+ \sum_{\substack{i,j \in [n-1] \\ i \neq j }}\Big[\big[|H(j \lor n)| - |H(i \lor j)|\big]\mathbb{I} _{ij > jn} \\&+ \big[|H(n \lor i)| - |H(i \lor j)|\big]\mathbb{I} _{ij > ni}\\ 
&+ \big[|H(j \lor n)| - |H(n \lor i)|\big]\mathbb{I} _{ni > jn}\\ &+ \big[|H(i \lor j)| - |H(n \lor i)|\big]\mathbb{I} _{ni > ij} \\ &+ \big[|H(n \lor i)| - |H(j \lor n)|\big]\mathbb{I} _{jn > ni}\\ &+ \big[|H(i \lor j)| - |H(j \lor n)|\big]\mathbb{I} _{nj > ij}\Big]\\
&= \sum_{\substack{i,j \in [n-1] \\ i \neq j }}|H(i \lor j)|\sum_{\substack{k \in [n-1] \\ k \neq i,j }}\big[\mathbb{I} _{ki > ij} - \mathbb{I} _{ij > ki} + \mathbb{I} _{jk > ij} - \mathbb{I} _{ij > jk}\big]\\
&+ \sum_{\substack{i,j \in [n-1] \\ i \neq j }}\Big[|H(i \lor j)|\big[\mathbb{I} _{jn > ij} - \mathbb{I} _{ij > jn} + \mathbb{I} _{ni > ij} - \mathbb{I} _{ij > ni}\big]\\ 
&+ |H(j \lor n)|\big[\mathbb{I} _{ij > jn} - \mathbb{I} _{jn > ij} + \mathbb{I} _{ni > jn} - \mathbb{I} _{jn > ni}\big]\\
&+ |H(n \lor i)|\big[\mathbb{I} _{jn > ni} - \mathbb{I} _{ni > jn} + \mathbb{I} _{ij > ni} - \mathbb{I} _{ni > ij}\big]\Big]\\
&= \sum_{\substack{i,j \in [n-1] \\ i \neq j }}|H(i \lor j)|\sum_{\substack{k \in [n] \\ k \neq i,j }}\big[\mathbb{I} _{ki > ij} - \mathbb{I} _{ij > ki} + \mathbb{I} _{jk > ij} - \mathbb{I} _{ij > jk}\big]\\
&+ \sum_{\substack{i,j \in [n-1] \\ i \neq j }} \Big[|H(j \lor n)|\big[\mathbb{I} _{ij > jn} - \mathbb{I} _{jn > ij} + \mathbb{I} _{ni > jn} - \mathbb{I} _{jn > ni}\big]\\
&+ |H(n \lor i)|\big[\mathbb{I} _{jn > ni} - \mathbb{I} _{ni > jn} + \mathbb{I} _{ij > ni} - \mathbb{I} _{ni > ij}\big]\Big]
\end{align*}
The term $ \sum_{\substack{i,j \in [n-1] \\ i \neq j }} \Big[|H(j \lor n)|\big[\mathbb{I} _{ij > jn} - \mathbb{I} _{jn > ij} + \mathbb{I} _{ni > jn} - \mathbb{I} _{jn > ni}\big]
+ |H(n \lor i)|\big[\mathbb{I} _{jn > ni} - \mathbb{I} _{ni > jn} + \mathbb{I} _{ij > ni} - \mathbb{I} _{ni > ij}\big]\Big] $ can be also represented as
\begin{align*}
&\sum_{\substack{i \in [n-1], j=n }} |H(i \lor j)|\sum_{\substack{k \in [n], k \neq i,j }}\big[\mathbb{I} _{ij > jk} - \mathbb{I} _{jk > ij} + \mathbb{I} _{ki > jk} - \mathbb{I} _{jk > ki}\big] +\\
& \sum_{\substack{j \in [n-1], i=n }}|H(i \lor j)|\sum_{\substack{k \in [n], k \neq i,j }}\big[\mathbb{I} _{jk > ki} - \mathbb{I} _{ki > jk} + \mathbb{I} _{ij > ki} - \mathbb{I} _{ki > ij}\big]
\end{align*}
Thus revenue for a tree with $n$ nodes is:
\begin{align*}
&Trev_{n}(H,[n]) =\\ &\sum_{\substack{i,j \in [n-1] \\ i \neq j }}|H(i \lor j)|\sum_{\substack{k \in [n] \\ k \neq i,j }}\big[\mathbb{I} _{ki > ij} - \mathbb{I} _{ij > ki} + \mathbb{I} _{jk > ij} - \mathbb{I} _{ij > jk}\big] +\\
& \sum_{\substack{i \in [n-1], j=n }} |H(i \lor j)|\sum_{\substack{k \in [n] \\ k \neq i,j }}\big[\mathbb{I} _{ij > jk} - \mathbb{I} _{jk > ij} + \mathbb{I} _{ki > jk} - \mathbb{I} _{jk > ki}\big] +\\
& \sum_{\substack{j \in [n-1], i=n }}|H(i \lor j)|\sum_{\substack{k \in [n] \\ k \neq i,j }}\big[\mathbb{I} _{jk > ki} - \mathbb{I} _{ki > jk} + \mathbb{I} _{ij > ki} - \mathbb{I} _{ki > ij}\big]\\
&= \sum_{\substack{i,j \in [n] \\ i \neq j }}|H(i \lor j)|\sum_{\substack{k \in [n] \\ k \neq i,j }}\big[\mathbb{I} _{ik > ij} - \mathbb{I} _{ij > ik} + \mathbb{I} _{jk > ij} - \mathbb{I} _{ij > jk}\big]\\
&= \sum_{\substack{i,j \in [n] \\ i \neq j }}|H(i \lor j)|(-s^{AddS3}_{ij}) = -Dcost(H,s^{AddS3})
\end{align*}


\section{Incomplete, incorrect proof of Proposition 2}

We prove Proposition \ref{thm-H0-maxrev} mainly by induction on $n$. 
\\ \textbf{Inductive hypothesis.} 
For any $k<n$, if $H_0$ is a binary tree on $[k]$ and $\mathcal{T}_0$ is induced by $H_0$, then $H_0 = \argmax_{H} Trev(H,\mathcal{T}_0)$.

For $n=1,2$ the statement is vacuous since there are no triplets. The base cases $n=3$ and 4 can be verified by enumerating all possible trees (we skip the details of this).
%
Before presenting the induction, we define the restriction of a tree $H$ and triplet set $\mathcal{T}$, and state few properties.

\begin{definition}[\textbf{Restriction of tree}]
Let $H$ be a tree on $[n]$. For any set $C \subseteq [n]$, the restriction of $H$ to $C$, denoted by $H_{|C}$ is a binary tree on $C$ obtained by removing all leaves not in $C$, removing all internal nodes without children and contracting all nodes with a single child.
\end{definition}

\begin{definition}[\textbf{Restriction of triplet set}]
Let $\mathcal{T}$ be a set of triplets on $[n]$. The restriction of $\mathcal{T}$ on the set $C \subseteq [n]$ is defined as the set $\mathcal{T}_{|C} = \{(i,j,k) \in \mathcal{T} ~:~ i,j,k \in C\} \subseteq \mathcal{T}$.
\end{definition}

The following is a restatement of \cite[][Proposition 2.1]{emamjomeh2018adaptive}.
\begin{lemma}
\label{lem-restriction}
Let $H_0$ be a binary tree on $[n]$ that induces the triplets $\mathcal{T}_0$.
For any $C \subseteq [n]$, let the restrictions $H_{0|C}$ and $\mathcal{T}_{0|C}$ be defined as above.
\begin{enumerate}
    \item $\mathcal{T}_{0|C}$ is the set of triplets induced by $H_{0|C}$;
    \item $H_{0|C}$ is the unique tree that satisfies all triplets in $\mathcal{T}_{0|C}$.
\end{enumerate}
\end{lemma}

We now present the arguments for induction, split into multiple parts.

\subsection{Part 1: Decomposition of $Trev$ for split at root node}

We aim to show that the latent tree $H_0$ maximises $Trev(H,\mathcal{T}_0)$. 
Assume that $H_0$ partitions the root node $[n]$ into the sets $A_1,A_2$.
On the other hand, assume that the maximiser $\widehat{H} = \argmax_H Trev(H,\mathcal{T}_0)$ partitions the root into $B_1,B_2$.
Further, define the sets $C_1 = A_1 \cap B_1$,  $D_1 = A_1 \cap B_2$, $C_2 = A_2 \cap B_1$,  $D_2 = A_2 \cap B_2$, that is, with respect to $H_0$, $\widehat{H}$ moves the objects in $D_1,D_2$ to the other child.

In Table \ref{tab-Trev}, we decompose the expression of $Trev(H,\mathcal{T}_0)$ for any tree $H$ into the contribution of triplets in $\mathcal{T}_{0|B_1}$, triplets in $\mathcal{T}_{0|B_2}$ and other terms.
We make a further simplification by renaming the indices $j,k$ for the case $(i,j,k) \in B_1\times B_1 \times B_2$ and the case $(i,j,k) \in B_2\times B_2 \times B_1$. The simplified expression is particularly useful since for every $i \in [n]$:
\begin{itemize}
    \item either $(i,j,k) \in \mathcal{T}_0$;
    \item or $(i,k,j) \in \mathcal{T}_0$;
    \item or neither of above are in $\mathcal{T}_0$, if $j,k$ are merged before $i$ in $H_0$.
\end{itemize}

We primarily interested in comparing the revenue for the the latent tree $H_0$ and the maximiser $\widehat{H}$.
In Table \ref{tab-Trev}, we simplify the expression for the revenue for $\widehat{H}$ by noting that $\widehat{H}$ splits the root into $B_1,B_2$, which implies:
\begin{itemize}
    \item when $(i,k) \in B_1\times B_2$ or $(i,k) \in B_2\times B_1$, then $|H(i\vee k)| = n$; and
    \item the case $i\in B_1; j,k \in B_2$ or $i\in B_2; j,k \in B_1$ have no contribution as $|H(i\vee k)| = |H(i\vee j)| = n$.
\end{itemize}

Finally Table \ref{tab-Trev} shows a lower bound for the revenue of $H_0$---a lower suffices here since showing that the lower bound is at least ar high as the revenue of $\widehat{H}$ would conclude that $H_0$ is a maximiser.
The lower bound stems from the fact that we drop the summations over $i\in B_1; j,k \in B_2$ and  $i\in B_2; j,k \in B_1$ since, by definition, $|H_0(i\vee k) \geq |H_0(i\vee j)|$ for all $(i,j,k)\in \mathcal{T}_0$.
Hence, we are left with the revenues with respect to $\mathcal{T}_{0|B_1}$ and $\mathcal{T}_{0|B_2}$, and the cross-terms involving $(i,j,k)\in B_1\times B_1\times B_2$ and $(i,j,k)\in B_2\times B_2\times B_1$.
Recall that $B_1 = C_1 \cup D_2$ and $B_2 = C_2 \cup D_1$, where the sets $C_1,C_2,D_1,D_2$ are defined earlier (recall $D_1,D_2$ denote the swapped sets).
Using this, we further decompose the cross-terms and note the $|H_0(i\vee j)|$ or $|H_0(i \vee k)|$ equal $n$, whenever the merger happens at the root of $H_0$ (for instance, $|H(i\vee k)|=n$ for $i \in C_1 \subseteq A_1$ and $k\in C_2 \subseteq A_2$).
We note here that since $i,j \in B_1; k \in B_2$ or vice-versa, the decomposition should lead to 16 cross-terms. But four cross terms do not induce triplets in $T_0$ since $j,k$ are merged before $i$ (for instance, $i\in C_1 \subseteq A_1; j \in D_2 \subseteq A_2; k \in C_2 \subseteq A_2$). 


\begin{table*}
\caption{Expression of $Trev(H,\mathcal{T}_0)$. ($B_1, B_2$ denotes a partition of $n$. For each sum, it is assumed that $i,j,k$ are distinct.)}
\label{tab-Trev}
\hrulefill

\textbf{For arbitrary tree $H$:}
\begin{align*}
Trev&(H,\mathcal{T}_0)
\\=& \sum_{\substack{i,j,k \in B_1 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
+ \sum_{\substack{i,j,k \in B_2 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
\\
&+ \sum_{i \in B_1} \left[ \sum_{\substack{j,k \in B_2 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
+ \sum_{\substack{j\in B_1, k \in B_2 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
+ \sum_{\substack{j\in B_2, k \in B_1 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
\right] 
\\
&+ \sum_{i \in B_2} \left[ \sum_{\substack{j,k \in B_1 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
+ \sum_{\substack{j\in B_2, k \in B_1 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
+ \sum_{\substack{j\in B_1, k \in B_2 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
\right] 
\\
=& ~Trev(H,\mathcal{T}_{0|B_1}) + Trev(H,\mathcal{T}_{0|B_2})
\\
&+ \sum_{i \in B_1} \left[ \sum_{\substack{j,k \in B_2 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
+ \sum_{j\in B_1, k \in B_2} (|H(i\vee k)| - |H(i\vee j)|) (\mathbb{I}_{(i,j,k) \in \mathcal{T}_0}
- \mathbb{I}_{(i,k,j) \in \mathcal{T}_0})
\right] 
\\
&+ \sum_{i \in B_2} \left[ \sum_{\substack{j,k \in B_1 \\ (i,j,k) \in \mathcal{T}_0}} (|H(i\vee k)| - |H(i\vee j)|)
+ \sum_{j\in B_2, k \in B_1} (|H(i\vee k)| - |H(i\vee j)|) (\mathbb{I}_{(i,j,k) \in \mathcal{T}_0}
- \mathbb{I}_{(i,k,j) \in \mathcal{T}_0})
\right] 
\end{align*}
\hrulefill

\textbf{For tree $\widehat{H}$ that splits root into $B_1,B_2$:}
\begin{align*}
Trev&(\widehat{H},\mathcal{T}_0)
\\
=& ~Trev(\widehat{H},\mathcal{T}_{0|B_1}) + Trev(\widehat{H},\mathcal{T}_{0|B_2})
\\
&+ \sum_{i \in B_1} 
\sum_{\substack{j\in B_1\\ k \in B_2}} (n - |H(i\vee j)|) (\mathbb{I}_{(i,j,k) \in \mathcal{T}_0}
- \mathbb{I}_{(i,k,j) \in \mathcal{T}_0})
+ \sum_{i \in B_2} \sum_{\substack{ j\in B_2\\ k \in B_1}} (n - |H(i\vee j)|) (\mathbb{I}_{(i,j,k) \in \mathcal{T}_0}
- \mathbb{I}_{(i,k,j) \in \mathcal{T}_0})
\end{align*}
\hrulefill

\textbf{Lower bound for latent tree $H_0$:}
\begin{align*}
Trev&(H_0,\mathcal{T}_0)
\\
\geq& ~Trev(H_0,\mathcal{T}_{0|B_1}) + Trev(H_0,\mathcal{T}_{0|B_2})
\\
&+ \sum_{i \in B_1} 
\sum_{\substack{j\in B_1\\ k \in B_2}} (|H_0(i\vee k)| - |H_0(i\vee j)|) (\mathbb{I}_{(i,j,k) \in \mathcal{T}_0}
- \mathbb{I}_{(i,k,j) \in \mathcal{T}_0})
+ \sum_{i \in B_2} \sum_{\substack{ j\in B_2\\ k \in B_1}} (|H_0(i\vee k)| - |H_0(i\vee j)|) (\mathbb{I}_{(i,j,k) \in \mathcal{T}_0}
- \mathbb{I}_{(i,k,j) \in \mathcal{T}_0})
\\
=& ~Trev(H_0,\mathcal{T}_{0|B_1}) + Trev(H_0,\mathcal{T}_{0|B_2})
\\
&+ \sum_{i\in C_1} \left[ \sum_{\substack{j \in C_1 \\ k \in C_2}} (n - |H_0(i\vee j)|)
+ \sum_{\substack{j \in C_1 \\ k \in D_1}} \big| |H_0(i\vee k)| - |H_0(i\vee j)| \big|
+ \sum_{\substack{j \in D_2 \\ k \in D_1}} (n - |H_0(i\vee k)|) \right]
\\
&+ \sum_{i \in D_2} \left[\sum_{\substack{j \in C_1 \\ k \in C_2}} (n - |H_0(i\vee k)|)
+ \sum_{\substack{j \in D_2 \\ k \in C_2}} \big| |H_0(i\vee k)| - |H_0(i\vee j)| \big|
+ \sum_{\substack{j \in D_2 \\ k \in D_1}} (n - |H_0(i\vee j)|) \right]
\\
&+ \sum_{i\in C_2} \left[ \sum_{\substack{j \in C_2 \\ k \in C_1}} (n - |H_0(i\vee j)|)
+ \sum_{\substack{j \in C_2 \\ k \in D_2}} \big| |H_0(i\vee k)| - |H_0(i\vee j)| \big|
+ \sum_{\substack{j \in D_1 \\ k \in D_2}} (n - |H_0(i\vee k)|) \right]
\\
&+ \sum_{i \in D_1} \left[\sum_{\substack{j \in C_2 \\ k \in C_1}} (n - |H_0(i\vee k)|)
+ \sum_{\substack{j \in D_1 \\ k \in C_1}} \big| |H_0(i\vee k)| - |H_0(i\vee j)| \big|
+ \sum_{\substack{j \in D_1 \\ k \in D_2}} (n - |H_0(i\vee j)|) \right]
\end{align*}
\hrulefill
\end{table*}

\subsection{Part 2: Proof of $Trev(\widehat{H}, \mathcal{T}_{0|B_1})\leq Trev(H_0, \mathcal{T}_{0|B_1})$}

Our aim is to show that $Trev(\widehat{H}, \mathcal{T}_{0})\leq Trev(H_0, \mathcal{T}_{0})$. We achieve this by first proving the inequality for the revenue with the restricted triplet sets $\mathcal{T}_{0|B_1},\mathcal{T}_{0|B_2}$ (this part), and the inequality for the sum of the cross terms (next part).

We prove only $Trev(\widehat{H}, \mathcal{T}_{0|B_1})\leq Trev(H_0, \mathcal{T}_{0|B_1})$ since the proof for $B_2$ follows similarly.
Recall that for every $(i,j,k) \in \mathcal{T}_0$, 
$|H_0(i\vee k)| > |H_0(i\vee j)|$, but the gap may reduce if we restrict the tree to $H_{0|C}$ for some set $C\subseteq [n]$, that is, for every $(i,j,k)\in \mathcal{T}_0$,
\[ |H_{0}(i \vee k)| - |H_{0}(i \vee j)| \geq 
|H_{0|C}(i \vee k)| - |H_{0|C}(i \vee j)|.\]
Hence, we have $Trev(H_{0},\mathcal{T}_{0|B_1}) \geq Trev(H_{0|B_1}, \mathcal{T}_{0|B_1})$.

On the other hand, note that $B_1$ is the left child of root of $\widehat{H}$. Hence, with respect to the triplets in $\mathcal{T}_{0|B_1}$, the revenue of $\widehat{H}$ and its restriction $\widehat{H}_{|B_1}$ are identical as there is no interaction with the right sub-tree of $\widehat{H}$. Thus, $Trev(\widehat{H},\mathcal{T}_{0|B_1}) = Trev(\widehat{H}_{|B_1}, \mathcal{T}_{0|B_1})$.

From Lemma \ref{lem-restriction}, we know that $H_{0|B_1}$ is the unique latent tree that induces $\mathcal{T}_{0|B_1}$, and our inductive hypothesis implies that $H_{0|B_1} = \argmax\limits_H Trev(H,\mathcal{T}_{0|B_1})$ since $|B_1| < n$.
Here, the maximum is over all binary trees on $B_1$, which also includes $\widehat{H}_{|B_1}$.
In particular, the optimality of $H_{0|B_1}$, combined with the above discussion, implies that
\begin{align*}
    Trev(H_0,\mathcal{T}_{0|B_1})
    &\geq Trev(H_{0|B_1},\mathcal{T}_{0|B_1})
    \\&\geq Trev(\widehat{H}_{|B_1},\mathcal{T}_{0|B_1})
    \\&=Trev(\widehat{H},\mathcal{T}_{0|B_1}),
\end{align*}
which proves the claim of this part.
The same arguments show that $Trev(H_0,\mathcal{T}_{0|B_1}) \geq Trev(\widehat{H},\mathcal{T}_{0|B_1})$.

\subsection{Part 3: Bounding the cross terms in the difference $Trev(H_0,\mathcal{T}_0) - Trev(\widehat{H}, \mathcal{T}_0)$}

We now prove that the contribution of the cross terms in the revenue of $H_0$, induced by $i,j \in B_1= C_1\cup D_2; k \in B_2 = C_2 \cup D_1$ or by $i,j \in B_2= C_2\cup D_1; k \in B_1 = C_1 \cup D_2$, exceed their contribution in the revenue of $\widehat{H}$.
Table \ref{tab} presents the cross terms for $H_0$ and the same can be computed for $\widehat{H}$. 
We note here that the four cases---$i\in C_1; j \in D_2; k \in C_2$ and similar three cases---that did not contribute in the revenue of $H_0$ also do not contribute to the revenue of $\widehat{H}$ since there are no corresponding triplets in $\mathcal{T}_0$.
In Table \ref{tab-Trev-diff}, we list the contribution of each 

\begin{table*}
\centering
\caption{Contribution of each case of $i,j,k$ in the difference $Trev(H_0,\mathcal{T}_0) - Trev(\widehat{H}, \mathcal{T}_0)$. The table only shows the 8 cases involving $i,j \in B_1 = C_1\cup D_2$ and $k \in B_2 = C_2 \cup D_1$. The other 8 cases can be computed in a symmetric way.}

\renewcommand{\arraystretch}{1.5}
\label{tab-Trev-diff}
\begin{tabular}{|c||c|c|}
    \hline
    & $k \in C_2$ & $k \in D_1$ \\
     \hline \hline
    \multirow{3}{*}{$i,j \in C_1$} 
    & $(n- |H_0(i\vee j)|) - (n-|H(i\vee j)|)$ 
    & $\big((|H_0(i\vee k)| - |H_0(i\vee j)|) - (n - |H(i\vee j)|)\big) $
    \\
    & $= |H(i\vee j)| - |H_0(i\vee j)|$
    & $\times (\mathbb{I}_{(i,j,k) \in \mathcal{T}_0}
- \mathbb{I}_{(i,k,j) \in \mathcal{T}_0})$
    \\ 
    & (cancels out when summed over $i,j\in C_1$)
    & $\geq |H(i\vee j)| - n$ \\
    \hline
    \multirow{2}{*}{$i \in C_1, j \in D_2$} 
    & \multirow{2}{*}{0}
    & $(n- |H_0(i\vee k)|) - (|H(i\vee j)|-n)$ \\
    & & $\geq 2n- |A_1| - |B_1|$\\
    \hline
    \multirow{2}{*}{$i \in D_2, j \in C_1$} 
    & $(n- |H_0(i\vee k)|) - (|H(i\vee j)|-n)$
    &  \multirow{2}{*}{0} \\
    & $\geq 2n- |A_2| - |B_1|$
    & \\
    \hline
    \multirow{3}{*}{$i, j \in D_2$} 
    & $\big((|H_0(i\vee k)| - |H_0(i\vee j)|) - (n - |H(i\vee j)|)\big) $
    & $(n- |H_0(i\vee j)|) - (n-|H(i\vee j)|)$ \\
    & $\times (\mathbb{I}_{(i,j,k) \in \mathcal{T}_0}
- \mathbb{I}_{(i,k,j) \in \mathcal{T}_0})$
    & $= |H(i\vee j)| - |H_0(i\vee j)|$
    \\
    & $\geq |H(i\vee j)| - n$ & 
    (cancels out when summed over $i,j\in D_2$)\\
    \hline
\end{tabular}
\end{table*}
\renewcommand{\arraystretch}{1}

